PASGAL: Parallel And Scalable Graph Algorithm Library

In this paper, we introduce PASGAL (Parallel And Scalable Graph Algorithm Library), a parallel graph library that scales to a variety of graph types, many processors, and large graph sizes. One special focus of PASGAL is the efficiency on \textit{large-diameter graphs}, which is a common challenge for many existing parallel graph processing systems: many existing graph processing systems can be even slower than the standard sequential algorithm on large-diameter graphs due to the lack of parallelism. Such performance degeneration is caused by the high overhead in scheduling and synchronizing threads when traversing the graph in the breadth-first order. The core technique in PASGAL to achieve high parallelism is a technique called \textit{vertical granularity control (VGC)} to hide synchronization overhead, as well as careful redesign of parallel graph algorithms and data structures. In our experiments, we compare PASGAL with state-of-the-art parallel implementations on BFS, SCC, BCC, and SSSP. PASGAL achieves competitive performance on small-diameter graphs compared to the parallel baselines, and is significantly faster on large-diameter graphs.

==> demo.tex <==
\section{Demostration Walkthrough}

==> intro-old.tex <==
\section{Introduction} 

Graphs are effective representations of real-world objects and their relationships in almost all areas in computer science. 
%such as social network users and their friendship,
%webpages and their links, geological objects and roads between them, machine learning objects and their similarities, etc. 
Processing and analyzing graphs efficiently have become increasingly important.
%One of the most important recent hardware advance that has impacted graph processing is the popularization of \emph{multicore systems.}
Given the large size of today's real-world graphs, it is imperative to consider parallelism in graph processing.
The increasing number of cores and memory size
allows a single machine to easily process graphs with billions of vertices in a few seconds,
even for reasonably complicated tasks.
As a result, a huge number of in-memory graph processing algorithms and systems have been developed (to list a few~\cite{}).
%Such parallel systems are applicable on from desktop PC (usually 4-16 processors) to high-end servers (hundreds of processors or more),
%and the number of core keeps increasing. 

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/bcc.pdf}
  \caption{\small Speedup on \#processors for biconnectivity algorithms over Hopcroft-Tarjan~\cite{hopcroft1973algorithm} (sequential, always 1).  
  \normalfont 
  The tested algorithms includes \pasgal{} (this paper), GBBS~\cite{gbbs2021}, Tarjan-Vishkin (TV)~\cite{tarjan1985efficient},
  and SM'14~\cite{}. 
  We present four graphs of different types. The top two graphs has small diameters and the bottom two has larger diameters.
  The largest graph Hyperlink14~\cite{webgraph} has 1.7 billion vertices. 
   \label{fig:bcc}}\label{fig:intro}
   \hide {GBBS~\cite{gbbs2021} 
  does not scale on some graphs due to theoretical inefficiency.  Tarjan-Vishkin~\cite{tarjan1985efficient} always scales (due to good span bound) but cannot run on large graphs (HL14~\cite{webgraph} has 1.7 billion vertices).  Due to theoretical efficiency, our algorithm~\cite{dong2023provably} is the fastest on all 27 tested graphs and always scales.
  }
\end{figure}

%Although the progress in hardware advance seems promising,
Despite the hardware advances, 
the increasing number of cores does not provide ``free'' performance improvement. 
We observed that many existing parallel software suffer from scalability issues, both to more cores and to larger/more diverse graphs,
even in fundamental tasks such as breadth-first search (BFS), strongly connected components (SCC), biconnected components (BCC), 
single source shortest paths (SSSP), etc.
We show an example of BCC algorithms in \cref{fig:intro}.
Tested on a 96-core machine,
many existing systems scale well with fewer than 16 threads and/or on the small-diameter graphs~\cite{}, 
but the performance can stop increasing (or even drop) with more threads, especially on large-diameter graphs.
On certain graphs, they can perform worse than a sequential algorithm. 
%Similar issues on other graph problems can be observed in \cref{fig:results}. 

We identified two major reasons for such performance degeneration: 
high overhead of managing and synchronizing threads, 
and/or space inefficiency.
While enabling the potential of better parallelism, more available cores also bring up great challenges and overhead.
Namely, \emph{parallelism comes at a cost}.
This is more pronounced on
using BFS-like primitives on large-diameter graphs:
when traversing the graph in BFS order, the number of rounds (and thus the synchronization cost) 
is proportional to graph diameter. 
Meanwhile, some existing systems do not scale to large data not because of time, but space.  
%Although multicore parallelism avoids the network latencies as in distributed systems and cloud computing, it is highly limited by its valuable main memory size.
Memory is the most valuable resource for in-memory graph processing systems. 
Hence, space-inefficient algorithms may only process graphs with small to medium size, making the improvement from parallelism much narrower.
This can also be seen by \cref{fig:intro}: \gbbs{} incurs high synchronization cost due to the use of BFS, 
leading to unsatisfactory performance on large-diameter graphs. 
Tarjan-Vishkin avoids using BFS by introducing high space overhead, and does not scale to billion-scale graphs. 

In this paper, we propose \emp{\pasgal} (Parallel and Scalable Graph Algorithm Library),
a graph processing library that is scalable to diverse graph types, many processors, and large graphs. 
We select several problems where high synchronization cost and/or space-inefficiency
can severely harm performance, including BFS, SCC, BCC, SSSP, etc., and plan to add more in the future.

To overcome the scalability issues, \pasgal{} employs three key techniques. 
The first is algorithm redesign to avoid using BFS. 
The second is a technique called \emph{vertical granularity control (VGC)} to hide scheduling overhead. 
%We further apply the idea to parallel BFS and achieved a new BFS implementation in \pasgal{}, which greatly improves the performance of BFS on large-diameter graphs. 
Finally, some new parallel data structures are used to facilitate the algorithms. 
In \cref{sec:algo}, we introduce our techniques in more details. 

With these techniques, \pasgal{} achieves high performance on a wide range of graphs, especially on large-diameter graphs.
We test various types of graphs, include very large graphs with billions of vertices. 
For the aforementioned BCC problem, \pasgal{} uses the FAST-BCC algorithm~\cite{},
which has strong theoretical guarantee in space and span (see details in \cref{sec:bcc}).
As shown in \cref{fig:intro}, \pasgal{} exhibits good scalability. 
%On SCC, BFS and SSSP, 
Overall, compared to the baselines, \pasgal{} is always competitive on small-diameter graphs, and is almost always the fastest on large diameter graphs. 
We discuss experimental results in \cref{sec:exp}. 
We provide the anonymous code~\cite{}, and plan to release it if the paper is accepted. 
Full experimental results and more references are given in the supplemental material. 
%Finally, we discuss other algorithms we plan to add in the future in \cref{sec:discussion}.

 


\hide{While reasons contribute to such performance degeneration,
a common issue that appears in multiple problems is the high synchronization cost.
%While bringing potential of better parallelism, more available processors also brings up great challenges and overhead.
Although more available processors offer the potential for improved parallelism, they also introduce significant challenges and increased overhead.
Namely, parallelism comes with a cost. }



%Many reasons contribute to such performance degeneration, such as the use of locks, insufficient parallelism (the existence of a long unparallelizable dependency chain in the algorithm), and the overhead of managing and synchronizing more threads.
%The goal of the proposed project is to enable high performance and scalability in processing large-scale graphs with a wide range of graphs.


==> lib.tex <==


